Learning Generalized Policies Without Supervision Using GNNs

We consider the problem of learning generalized policies for classical planning domains using graph neural networks from small instances represented in lifted STRIPS. The problem has been considered before but the proposed neural architectures are complex and the results are often mixed. In this work, we use a simple and general GNN architecture and aim at obtaining crisp experimental results and a deeper understanding: either the policy greedy in the learned value function achieves close to 100% generalization over instances larger than those used in training, or the failure must be understood, and possibly fixed, logically. For this, we exploit the relation established between the expressive power of GNNs and the $C_{2}$ fragment of first-order logic (namely, FOL with 2 variables and counting quantifiers). We find for example that domains with general policies that require more expressive features can be solved with GNNs once the states are extended with suitable "derived atoms" encoding role compositions and transitive closures that do not fit into $C_{2}$. The work follows the GNN approach for learning optimal general policies in a supervised fashion (Stahlberg, Bonet, Geffner, 2022); but the learned policies are no longer required to be optimal (which expands the scope, as many planning domains do not have general optimal policies) and are learned without supervision. Interestingly, value-based reinforcement learning methods that aim to produce optimal policies, do not always yield policies that generalize, as the goals of optimality and generality are in conflict in domains where optimal planning is NP-hard.

==> extensions-variations.tex <==
\section{Extensions and Variations}


\input{rl.tex}

\input{derived.tex}


==> linear-projections.tex <==
\subsection{Linear \CC Projections}

\begin{table*}[t]
    \centering
    \begin{tabular}{@{}lllllll@{}}
        \toprule
        Domain (\#)      & Coverage (\%) & L     & PQ = PL / OL (\#)        & \# F & $k$   & MC \\
        \midrule
        \gripper{} (16)  & 16 (100\%)    & 3864  & 1.091 = 192 / 176 (4)    & 16   & 31458 & 14 \\
        \miconic{} (120) & 112 (93\%)    & 16634 & 2.154 = 2372 / 1101 (33) & 30   & 43254 & 10 \\
        \visitall{} (14) & 13 (93\%)     & 1050  & 1.690 = 720 / 426 (9)    & 25   & 31302 & 12 \\
        \midrule
        Total (150)      & 141 (94\%)    & 21548 & 1.928 = 3284 / 1703 (46)                     \\
        \bottomrule
    \end{tabular}
    \caption{
        Coverage is the number of solved problems in the test set when \textbf{???} on policy $\pi_V$ for learned $V$.
        In additions to the columns in Table~\ref{tbl:experiments:coverage},
        \# F refers to the number of features in \textbf{???},
        $k$ is the number of features in the pool,
        and MC is the maximum complexity in the pool.
    }
    \label{tbl:linearprojections:coverage}
\end{table*}



Value functions can also be expressed as linear combinations of description logic (DL) features~\citep{frances:ijcai2019}.
One benefit of this approach is that the features can be understood and checked for correctness.
In this section we show that such value functions can sometimes approximate our learned models.

The procedure is this.
Let $s_1, \dots, s_n$ be states, $V$ a learned model, and $f_1, \dots, f_k$ Boolean or numerical description logic features ($f(s) \in \{0, 1\}$ for Boolean features).
Also let $c_1, \dots, c_k$ be coefficients for the features.
Then the following equations are optimized w.r.t. squared error and $L_0$ regularization (minimize number of non-zero coefficients):
\[
    \begin{bmatrix}
        f_1(s_1) & \dots  & f_k(s_1) \\
        \vdots   & \ddots & \vdots \\
        f_1(s_n) & \dots  & f_k(s_n)
    \end{bmatrix}
    \begin{bmatrix}
        c_1 \\
        \vdots \\
        c_k
    \end{bmatrix}
    =
    \begin{bmatrix}
        V(s_1) \\
        \vdots \\
        V(s_n)
    \end{bmatrix}
\]

We used the software provided by~\citep{drexler-et-al-dlplan2022} to generate all description logic features, the CPU-time limit was set to $24$ hours on a Ryzen 9 5900X.
The software L0Learn~\citep{l0learn} was used for optimization.

Table~\ref{tbl:linearprojections:coverage} show that we were able to find $3$ policies expressed as linear functions of DL features that approximate our learned $V$ (trained with $L_3$) that also generalized well to the test set.
The absolute error for these domains were roughy: $0.2$ for Gripper and Miconic, and $0.5$ for VisitAll.
However, these policies are not transparent as they require between $16$ to $30$ features.
For the domains Blocks, Delivery, and Reward, we did not find a policy with a sufficiently low absolute error, this can happen if either: 1) the feature pool does not contain the correct features; or 2) a linear function of DL features cannot express the value function.
It is difficult to pinpoint the actual reason, but \citep{frances:ijcai2019} suggests that for the complexity of DL features need to be very high for Blocks and Logistics ($49$ and $22$, resp.).

\textbf{TODO: Define complexity of DL feature. Give examples?}


==> table1.tex <==
                                         blocks  (20) &  20 (100\%) &    790 &  1.0427 =    440 /    422  (13) &  20 (100\%) &    790 &  1.0427 =    440 /    422  (13) \\
                                       delivery  (15) &  15 (100\%) &    400 &  1.0000 =    400 /    400  (15) &  15 (100\%) &    404 &  1.0100 =    404 /    400  (15) \\
                                        gripper  (16) &  16 (100\%) &  1,286 &  1.0000 =    176 /    176   (4) &  16 (100\%) &  1,286 &  1.0000 =    176 /    176   (4) \\
                         logistics-max-v0-97564  (28) &  17  (60\%) &  4,635 &  9.7215 =  3,665 /    377  (15) &   0   (0\%) &      0 &                             --- \\
                                        miconic (120) & 120 (100\%) &  7,331 &  1.0052 =  1,170 /  1,164  (35) & 120 (100\%) &  7,331 &  1.0052 =  1,170 /  1,164  (35) \\
                                         reward  (15) &  11  (73\%) &  1,243 &  1.2306 =  1,062 /    863  (10) &   3  (20\%) &    237 &  1.1232 =    237 /    211   (3) \\
                          spanner-bidirectional  (41) &  30  (73\%) &  1,545 &  1.0000 =  1,545 /  1,545  (30) &  24  (58\%) &    940 &  1.0000 =    940 /    940  (24) \\
                                       visitall  (14) &  14 (100\%) &    904 &  1.0183 =    556 /    546  (10) &  11  (78\%) &    631 &  1.0107 =    471 /    466   (9) \\
\midrule
                                      blocks-L0  (20) &   0   (0\%) &      0 &                             --- &   0   (0\%) &      0 &                             --- \\
                                    delivery-L0  (15) &  12  (80\%) &    278 &  1.0000 =    278 /    278  (12) &   0   (0\%) &      0 &                             --- \\
                                     gripper-L0  (16) &  16 (100\%) &  1,288 &  1.0000 =    176 /    176   (4) &   0   (0\%) &      0 &                             --- \\
                                     miconic-L0 (120) & 120 (100\%) &  7,758 &  1.0241 =  1,192 /  1,164  (35) &   0   (0\%) &      0 &                             --- \\
                                      reward-L0  (15) &  12  (80\%) &  1,362 &  1.1226 =    861 /    767   (9) &   0   (0\%) &      0 &                             --- \\
                                    visitall-L0  (14) &  14 (100\%) &    838 &  1.0073 =    550 /    546  (10) &   0   (0\%) &      0 &                             --- \\
\midrule
               logistics-augmented-max-v1-35099  (28) &  21  (75\%) &  3,357 &  2.5295 =  1,156 /    457  (17) &   5  (17\%) &    117 &  1.0734 =    117 /    109   (5) \\
               logistics-augmented-max-v2-44459  (28) &  28 (100\%) &  5,548 &  3.0744 =  1,405 /    457  (17) &   0   (0\%) &      0 &                             --- \\
               logistics-augmented-max-v2-90154  (28) &  28 (100\%) &  8,147 &  5.5711 =  2,546 /    457  (17) &   4  (14\%) &     88 &  1.0353 =     88 /     85   (4) \\
\midrule
             spanner-bidirectional-max-v0-83399  (36) &  12  (33\%) &    557 &  1.0000 =    557 /    557  (12) &   8  (22\%) &    373 &  1.0000 =    373 /    373   (8) \\
          spanner-bidirectional-addmax-v0-18347  (36) &  29  (80\%) &  1,244 &  1.0017 =  1,178 /  1,176  (28) &   8  (22\%) &    222 &  1.0000 =    222 /    222   (8) \\
   spanner-bidirectional-augmented-max-v0-26687  (36) &  36 (100\%) &  1,606 &  1.0000 =  1,348 /  1,348  (32) &  36 (100\%) &  1,606 &  1.0000 =  1,348 /  1,348  (32) \\
   spanner-bidirectional-augmented-max-v1-73391  (36) &  31  (86\%) &  1,370 &  1.0000 =  1,112 /  1,112  (27) &  28  (77\%) &  1,190 &  1.0000 =    996 /    996  (25) \\
spanner-bidirectional-augmented-addmax-v1-30023  (36) &  34  (94\%) &  1,498 &  1.0000 =  1,240 /  1,240  (30) &  34  (94\%) &  1,503 &  1.0000 =  1,243 /  1,243  (30) \\
spanner-bidirectional-augmented-addmax-v2-88403  (36) &  31  (86\%) &  1,365 &  1.0016 =  1,233 /  1,231  (30) &  16  (44\%) &    603 &  1.0000 =    603 /    603  (16) \\
\midrule
                                          Total (769) & 667  (86\%) & 54,350 &  1.4488 = 23,846 / 16,459 (412) & 348  (45\%) & 17,321 &  1.0080 =  8,828 /  8,758 (231) \\

